Language Models with Image Descriptors are Strong Few-Shot Video-Language Learners

The goal of this work is to build flexible video-language models that can generalize to various video-to-text tasks from few examples, such as domain-specific captioning, question answering, and future event prediction. Existing few-shot video-language learners focus exclusively on the encoder, resulting in the absence of a video-to-text decoder to handle generative tasks. Video captioners have been pretrained on large-scale video-language datasets, but they rely heavily on finetuning and lack the ability to generate text for unseen tasks in a few-shot setting. We propose VidIL, a few-shot Video-language Learner via Image and Language models, which demonstrates strong performance on few-shot video-to-text tasks without the necessity of pretraining or finetuning on any video datasets. We use the image-language models to translate the video content into frame captions, object, attribute, and event phrases, and compose them into a temporal structure template. We then instruct a language model, with a prompt containing a few in-context examples, to generate a target output from the composed content. The flexibility of prompting allows the model to capture any form of text input, such as automatic speech recognition (ASR) transcripts. Our experiments demonstrate the power of language models in understanding videos on a wide variety of video-language tasks, including video captioning, video question answering, video caption retrieval, and video future event prediction. Especially, on video future event prediction, our few-shot model significantly outperforms state-of-the-art supervised models trained on large-scale video datasets. Code and resources are publicly available for research purposes at https://github.com/MikeWangWZHL/VidIL .

==> 9_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:ablation}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See supplemental material.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:experimental_setup} and  supplemental material. }
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{sec:ablation}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \answerYes{See Section~\ref{sec:experimental_setup}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{see Section~\ref{sec:ablation}.}
  \item Did you mention the license of the assets?
     \answerYes{see the citations in  Section~\ref{sec:ablation}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{see the citations in  Section~\ref{sec:ablation}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{see the citations in  Section~\ref{sec:ablation}. }
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> table/alpro_template.tex <==
\begin{table*}[htb]
    % \small
    % \vspace{1ex}
    % \aboverulesep = 0.55mm
    % \belowrulesep = 0.55mm
	\centering	
  % \setlength\tabcolsep{5pt}
% 	\resizebox{0.95\textwidth}{!}
	\resizebox{1.0\textwidth}{!}
{%
	\begin{tabular}	{l   c@{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}} c c @{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}} c @{\hspace{1.5\tabcolsep}}c
	@{\hspace{1.5\tabcolsep}}c
	@{\hspace{1.5\tabcolsep}}c 
	@{\hspace{1.5\tabcolsep}}c
	@{\hspace{1.5\tabcolsep}}c
	@{\hspace{1.5\tabcolsep}}c@{\hspace{1.5\tabcolsep}}}
		\toprule \multirow{2}{*}{\textbf{Pre-training tasks}} & \multicolumn{4}{c}{\footnotesize\textbf{MSRVTT Retrieval}}& \multicolumn{4}{c}{\footnotesize\textbf{DiDeMo Retrieval}} & \footnotesize\textbf{MSVD-QA} & \footnotesize\textbf{MSRVTT-QA} \\
	 &  \footnotesize\textbf{R1}$\uparrow$ &\footnotesize\textbf{ R5}$\uparrow$
	 &  \footnotesize\textbf{R10}$\uparrow$ &\footnotesize\textbf{ MdR}$\downarrow$
	 & \footnotesize \textbf{R1}$\uparrow$ & \footnotesize\textbf{R5}$\uparrow$
	 & \footnotesize\textbf{R10}$\uparrow$ & \footnotesize\textbf{MdR}$\downarrow$ & \footnotesize\textbf{Acc.}$\uparrow$ &  \footnotesize\textbf{Acc.}$\uparrow$\\
	 	 \midrule
      w/o pre-training & 16.5 & 42.8 & 57.9 & 7 & 9.5 & 29.1 & 42.5 & 14 & 41.5 & 39.6  \\
      MLM + VTM & 28.5 & 53.0 & 66.8 & 5 & 29.8 & 57.7 & 69.7 & 4 & 43.3 & 40.9 \\
      MLM + VTM + PEM & 30.3 & 56.7 & 67.8 & 4 & 31.0 & 61.8 & 73.5 & 3 &  \textbf{46.3} & 41.8 \\
      MLM + VTM + VTC & 32.8 & 59.2 & 70.3 & 3 & \textbf{36.8} & 64.7 & 77.4 & \textbf{2} & 45.5 & 41.9 \\
      MLM + VTM + PEM + VTC & \textbf{33.9} & \textbf{60.7} & \textbf{73.2} & \textbf{3} & 35.9 & \textbf{67.5} & \textbf{78.8} & 3 & 45.9  & \textbf{42.1} \\
	 
	
		\bottomrule
	\end{tabular}}
%	}
    \vspace{-5pt}
	\caption
	{Evaluations of the proposed pre-training objectives on four downstream datasets. MLM: masked language modeling loss. VTM: video-text matching loss. PEM: prompting entity modeling loss. VTC: video-text contrastive loss. 
	R@k denotes recall (\%) with k retrieval efforts; MdR denotes median ranking for retrieved videos. We use acc. to denote accuracy.
	}
	\label{tbl:main}
% 	\vspace{-2ex}

\end{table*}		
